A Hybrid Submodular Optimization Approach to Controlled Islanding with Post-Disturbance Stability Guarantees

Disturbances may create cascading failures in power systems and lead to widespread blackouts. Controlled islanding is an effective approach to mitigate cascading failures by partitioning the power system into a set of disjoint islands. To retain the stability of the power system following disturbances, the islanding strategy should not only be minimally disruptive, but also guarantee post-disturbance stability. In this paper, we study the problem of synthesizing post-disturbance stability-aware controlled islanding strategies. To ensure post-disturbance stability, our computation of islanding strategies takes load-generation balance and transmission line capacity constraints into consideration, leading to a hybrid optimization problem with both discrete and continuous variables. To mitigate the computational challenge incurred when solving the hybrid optimization program, we propose the concepts of hybrid submodularity and hybrid matroid. We show that the islanding problem is equivalent to a hybrid matroid optimization program, whose objective function is hybrid supermodular. Leveraging the supermodularity property, we develop an efficient local search algorithm and show that the proposed algorithm achieves 1/2-optimality guarantee. We compare our approach with a baseline using mixed-integer linear program on IEEE 118-bus, IEEE 300-bus, ActivSg 500-bus, and Polish 2383-bus systems. Our results show that our approach outperforms the baseline in terms of the total cost incurred during islanding across all test cases. Furthermore, our proposed approach can find an islanding strategy for large-scale test cases such as Polish 2383-bus system, whereas the baseline approach becomes intractable.

==> formulation.tex <==
\section{Islanding Formulation}\label{sec:formulation}

Our goal is to partition the power system $G$ into $m$ disjoint islands, denoted as $I_1,\ldots,I_m$, to mitigate cascading failures.
Each island $I_k$ can be represented as 
\begin{equation*}
    I_k=(\mathcal{V}_k,\mathcal{E}_k),
\end{equation*}
where $\mathcal{V}_k\subset\mathcal{V}$ is a subset of buses and $\mathcal{E}_k=(\mathcal{V}_k\times\mathcal{V}_k)\cap \mathcal{E}$ is a subset of transmission lines.
To ensure the islands to be disjoint, we have that $\mathcal{V}_k\cap\mathcal{V}_{k'}=\emptyset$ for all $k\neq k'$.
In addition, each island $I_k$ is connected for all $k=1,\ldots,m$.
Given the number of islands $m$, we select a collection of reference generators, denoted as $\{r_k:k=1,\ldots,m\}$.
We refer the readers to \cite{chow1982time} for methodologies of choosing reference generators.
For each reference generator $r_k$, it must be contained within island $I_k$ when partitioning the power system.
In the remainder of this paper, we will denote $E=\cup_{k=1}^m\mathcal{E}_k$ as the set of transmission lines that remain connected in the power system after formulating the islands.

In this paper, we partition the power system into $m$ number of islands by optimizing the following metrics: (i) load-generation balance, (ii) generator coherency, and (iii) power flow disruption. We formulate each metric in detail below.

Partitioning the power system into islands may cause violations of load-generation balance constraint given in Eqn. \eqref{eq:balance}. 
To ensure that load-generation balance constraint remains to be satisfied for each island, some loads from load buses need to be shed.
We define $c_j:\mathbb{R}\rightarrow\mathbb{R}$ as the cost function of load shedding for load bus $j$.
We assume that function $c_j$ is monotone increasing and convex.
Then given set $E$, the loads $d=[d_1,\ldots,d_{|\mathcal{L}|}]^\top$ attached to the load buses in $\mathcal{L}$ can be found by
\begin{subequations}\label{eq:island balance}
\begin{align}
    F_1(E,d) = &\min_d\quad\sum_{j\in\mathcal{L}}c_j(\Bar{d}_j-d_j)\\
    &\st\quad\sum_{j\in \mathcal{L}\cap \mathcal{V}_k} d_j\leq \sum_{j\in \mathcal{G}\cap \mathcal{V}_k} \Bar{g}_j,~\forall k=1,\ldots,m\label{eq:island balance-2}\\
    &\quad\quad\quad d_j\in[0,\Bar{d}_j],~\forall j\in\mathcal{L}.\label{eq:island balance-3}
\end{align}
\end{subequations}
Any feasible solution to optimization program \eqref{eq:island balance} guarantees that the total amount of loads $\sum_{j\in \mathcal{L}\cap \mathcal{V}_k} d_j$ within each island is less than the total power generation capacity $\sum_{j\in \mathcal{G}\cap \mathcal{V}_k} \Bar{g}_j$.
In the remainder of this paper, we define $(E,d)$ as an islanding strategy, which specifies the set of transmission lines that will remain in the system as well as the amount of load shedding incurred by the load buses.

% Given an islanding strategy $(E,d)$ and the generation capacity for each generator bus, the post-islanding power flow $\Tilde{P}_{jj'}$ on each transmission line $(j,j')\in E$ is determined by Eqn. \eqref{eq:conservation}. 
% To avoid further disrupting the power system, the post-islanding power flow needs to satisfy the capacity constraint $\Tilde{P}_{jj'}\leq \Bar{P}_{jj'}$ for all $(j,j')\in E$.

We next consider generator coherence. We denote the coherence matrix as $\Bar{A}\in\mathbb{R}^{m\times |\mathcal{G}|}$, which is independent of the islanding strategy (see \cite{chow1982time} for the detailed introduction on $\Bar{A}$). Then the generator coherence is computed as
\begin{equation}\label{eq:coherence}
    F_2(E) = \|\Bar{A}-A(E)\|_F,
\end{equation}
where $\|\cdot\|_F$ represents the Frobenius norm, and $A(E)\in\mathbb{R}^{|\mathcal{G}|\times m}$ whose $(j,k)$-th entry is defined as
\begin{equation*}
    \left[A(E)\right]_{jk} = \begin{cases}
    1,&\mbox{ if $j\in \mathcal{V}_k$},\\
    0,&\mbox{ otherwise}.
    \end{cases}
\end{equation*}

We finally describe the metric on power flow disruption. This metric measures the total amount of power flow being disrupted due to tripping transmission lines to form islands.
The power flow disruption can be computed as
\begin{equation}\label{eq:disruption}
    F_3(E) = \sum_{(j,j')\in\mathcal{E}\setminus E}\frac{|P_{jj'}|}{2}.
\end{equation}
We remark that the power flow $P_{jj'}$ in Eqn. \eqref{eq:disruption} is the pre-islanding power flow before forming the islands.

In addition to the metrics defined in Eqn. \eqref{eq:island balance}, \eqref{eq:coherence}, and \eqref{eq:disruption}, the islanding strategy should satisfy the following two constraints.
First, the post-islanding power flow, denoted as $\Tilde{P}_{jj'}$, should satisfy the conservation law given in Eqn. \eqref{eq:conservation}. Furthermore, the post-islanding power flow needs to satisfy the transmission line capacity constraint given as below
\begin{equation}\label{eq:island capacity}
    \Tilde{P}_{jj'}\leq \Bar{P}_{jj'}, ~(j,j')\in E,
\end{equation}
in order to ensure the post-islanding stability.
Finally, each island should contain at least one black start generator to ensure that the power system can be restored and reconnected. 
This constraint is formulated as follows
\begin{equation}\label{eq:blackstart}
    \sum_{j\in\mathcal{V}_k}\mathbb{I}_{j}\geq 1,~\forall k=1,\ldots,m
\end{equation}
where $\mathbb{I}_{j}$ is an indicator function defined as
\begin{equation*}
    \mathbb{I}_{j} = \begin{cases}
    1,&\mbox{if a black start generator is attached to $j$},\\
    0,& \mbox{otherwise}.
    \end{cases}
\end{equation*}

Let $\alpha_i\in[0,1]$ for $i=1,2,3$ be constants modeling the trade-off parameters among metrics $F_1(E,d)$, $F_2(E)$, and $F_3(E)$, respectively. 
We then formulate the following optimization program to compute the islanding strategy $(E,d)$
\begin{subequations}\label{eq:islanding formulation}
\begin{align}
    \min_{E,d} \quad&\alpha_1F_1(E,d)+\alpha_2F_2(E) + \alpha_3F_3(E)\\
    \st \quad & r_k\in I_k,~\forall k=1,\ldots,m\label{eq:ref gen}\\
    &\text{$I_1,\ldots,I_m$ form a set of islands}\label{eq:islanding validity constraint}\\
    &\text{Eqn. \eqref{eq:conservation}, \eqref{eq:island balance-2}, \eqref{eq:island balance-3}, \eqref{eq:island capacity}, and \eqref{eq:blackstart}}\label{eq:islanding constraint}
\end{align}
\end{subequations}




==> formulation_v2.tex <==
\section{System Model and Islanding Formulation}\label{sec:formulation}

We consider a power system and model it as a graph, denoted as $G=(\mathcal{V},\mathcal{E})$, where $\mathcal{V}$ is the set of vertices and $\mathcal{E}\subseteq\mathcal{V}\times\mathcal{V}$ is the set of edges. 
Without loss of generality, we assume that graph $G$ is connected.
Here we use the set of vertices $\mathcal{V}=\{1,\ldots,n\}$ to represent the set of buses, and use the set of edges $\mathcal{E}$ to represent the collection of transmission lines.
Among the buses, we denote the set of generator and load buses as $\mathcal{G}\subseteq \mathcal{V}$ and $\mathcal{L}\subseteq \mathcal{V}$, respectively, where $\mathcal{G}\cap\mathcal{L}=\emptyset$.
For each generator bus $j\in\mathcal{G}$, we denote its generation capacity as $\Bar{g}_j$. For each load bus $j\in\mathcal{L}$, we denote its maximum load as $\Bar{d}_j$. For each transmission line $(j,j')\in\mathcal{E}$, we denote the power flow from bus $j$ to $j'$ through transmission line $(j,j')$ as $P_{jj'}$. The power flow $P_{jj'}$ should be limited as $P_{jj'}\leq \Bar{P}_{jj'}$ to avoid overflow and transmission line outage. We denote $\Bar{P}_{jj'}$ as the transmission line capacity of $(j,j')$.

Our goal is to partition the power system $G$ into $m$ disjoint islands, denoted as $I_1,\ldots,I_m$, to mitigate cascading failures.
Each island $I_k$ can be represented as 
\begin{equation*}
    I_k=(\mathcal{V}_k,\mathcal{E}_k),
\end{equation*}
where $\mathcal{V}_k\subset\mathcal{V}$ is a subset of buses and $\mathcal{E}_k=(\mathcal{V}_k\times\mathcal{V}_k)\cap \mathcal{E}$ is a subset of transmission lines.
To ensure the islands to be disjoint, we have that $\mathcal{V}_k\cap\mathcal{V}_{k'}=\emptyset$ for all $k\neq k'$.
In addition, each island $I_k$ is connected for all $k=1,\ldots,m$.
Given the number of islands $m$, we select a collection of reference generators, denoted as $\{r_k:k=1,\ldots,m\}$.
We refer the readers to \cite{chow1982time} for methodologies of choosing reference generators.
For each reference generator $r_k$, it must be contained within island $I_k$ when partitioning the power system.
In the remainder of this paper, we will denote $E=\cup_{k=1}^m\mathcal{E}_k$ as the set of transmission lines that remain connected in the power system after formulating the islands.

In this paper, we partition the power system into $m$ number of islands by optimizing the following metrics: (i) load-generation balance, (ii) generator coherency, and (iii) power flow disruption. We formulate each metric in detail below.

Partitioning the power system into islands may cause violations of load-generation balance constraint given in Eqn. \eqref{eq:balance}. 
To ensure that load-generation balance constraint remains to be satisfied for each island, some loads from load buses need to be shed.
We define $c_j:\mathbb{R}\rightarrow\mathbb{R}$ as the cost function of load shedding for load bus $j$.
We assume that function $c_j$ is monotone increasing and convex.
Then given set $E$, the loads $d=[d_1,\ldots,d_{|\mathcal{L}|}]^\top$ attached to the load buses in $\mathcal{L}$ can be found by
\begin{subequations}\label{eq:island balance}
\begin{align}
    F_1(E,d) = &\min_d\quad\sum_{j\in\mathcal{L}}c_j(\Bar{d}_j-d_j)\\
    &\st\quad\sum_{j\in \mathcal{L}\cap \mathcal{V}_k} d_j\leq \sum_{j\in \mathcal{G}\cap \mathcal{V}_k} \Bar{g}_j,~\forall k=1,\ldots,m\label{eq:island balance-2}\\
    &\quad\quad\quad d_j\in[0,\Bar{d}_j],~\forall j\in\mathcal{L}.\label{eq:island balance-3}
\end{align}
\end{subequations}
Any feasible solution to optimization program \eqref{eq:island balance} guarantees that the total amount of loads $\sum_{j\in \mathcal{L}\cap \mathcal{V}_k} d_j$ within each island is less than the total power generation capacity $\sum_{j\in \mathcal{G}\cap \mathcal{V}_k} \Bar{g}_j$.
In the remainder of this paper, we define $(E,d)$ as an islanding strategy, which specifies the set of transmission lines that will remain in the system as well as the amount of load shedding incurred by the load buses.

% Given an islanding strategy $(E,d)$ and the generation capacity for each generator bus, the post-islanding power flow $\Tilde{P}_{jj'}$ on each transmission line $(j,j')\in E$ is determined by Eqn. \eqref{eq:conservation}. 
% To avoid further disrupting the power system, the post-islanding power flow needs to satisfy the capacity constraint $\Tilde{P}_{jj'}\leq \Bar{P}_{jj'}$ for all $(j,j')\in E$.

We next consider generator coherence. We denote the coherence matrix as $\Bar{A}\in\mathbb{R}^{m\times |\mathcal{G}|}$, which is independent of the islanding strategy (see \cite{chow1982time} for the detailed introduction on $\Bar{A}$). Then the generator coherence is computed as
\begin{equation}\label{eq:coherence}
    F_2(E) = \|\Bar{A}-A(E)\|_F,
\end{equation}
where $\|\cdot\|_F$ represents the Frobenius norm, and $A(E)\in\mathbb{R}^{|\mathcal{G}|\times m}$ whose $(j,k)$-th entry is defined as
\begin{equation*}
    \left[A(E)\right]_{jk} = \begin{cases}
    1,&\mbox{ if $j\in \mathcal{V}_k$},\\
    0,&\mbox{ otherwise}.
    \end{cases}
\end{equation*}

We finally describe the metric on power flow disruption. This metric measures the total amount of power flow being disrupted due to tripping transmission lines to form islands.
The power flow disruption can be computed as
\begin{equation}\label{eq:disruption}
    F_3(E) = \sum_{(j,j')\in\mathcal{E}\setminus E}\frac{|P_{jj'}|}{2}.
\end{equation}
We remark that the power flow $P_{jj'}$ in Eqn. \eqref{eq:disruption} is the pre-islanding power flow before forming the islands.

In addition to the metrics defined in Eqn. \eqref{eq:island balance}, \eqref{eq:coherence}, and \eqref{eq:disruption}, the islanding strategy should satisfy the following constraints.
First, the post-islanding power flow, denoted as $\Tilde{P}_{jj'}$, should satisfy the conservation law given as
\begin{equation}\label{eq:conservation}
    \sum_{j':(j,j')\in\mathcal{E}}P_{jj'}+ d_j - g_j = 0,~\forall j\in\mathcal{V}.
\end{equation}
Furthermore, the post-islanding power flow needs to satisfy the transmission line capacity constraint given as below
\begin{equation}\label{eq:island capacity}
    \Tilde{P}_{jj'}\leq \Bar{P}_{jj'}, ~(j,j')\in E,
\end{equation}
in order to ensure the post-islanding stability.
Finally, each island should contain at least one black start generator to ensure that the power system can be restored and reconnected. 
This constraint is formulated as follows
\begin{equation}\label{eq:blackstart}
    \sum_{j\in\mathcal{V}_k}\mathbb{I}_{j}\geq 1,~\forall k=1,\ldots,m
\end{equation}
where $\mathbb{I}_{j}$ is an indicator function defined as
\begin{equation*}
    \mathbb{I}_{j} = \begin{cases}
    1,&\mbox{if a black start generator is attached to $j$},\\
    0,& \mbox{otherwise}.
    \end{cases}
\end{equation*}

Let $\alpha_i\in[0,1]$ for $i=1,2,3$ be constants modeling the trade-off parameters among metrics $F_1(E,d)$, $F_2(E)$, and $F_3(E)$, respectively. 
We then formulate the following optimization program to compute the islanding strategy $(E,d)$
\begin{subequations}\label{eq:islanding formulation}
\begin{align}
    \min_{E,d} \quad&\alpha_1F_1(E,d)+\alpha_2F_2(E) + \alpha_3F_3(E)\\
    \st \quad & r_k\in I_k,~\forall k=1,\ldots,m\label{eq:ref gen}\\
    &\text{$I_1,\ldots,I_m$ form a set of islands}\label{eq:islanding validity constraint}\\
    &\text{Eqn. \eqref{eq:conservation}, \eqref{eq:island balance-2}, \eqref{eq:island balance-3}, \eqref{eq:island capacity}, and \eqref{eq:blackstart}}\label{eq:islanding constraint}
\end{align}
\end{subequations}




==> intro.tex <==
\section{Introduction}
\IEEEPARstart{P}{ower} systems nowadays are often operated at points closing to their limits.
As a consequence, when power systems incur disturbances such as cyber attacks \cite{case2016analysis}, natural disasters \cite{busby2021cascading}, and spiking growth in power demand \cite{pidd2012india}, some transmission lines and generators may incur outage, leading to overflow at neighboring transmission lines and hence cascading failures \cite{hines2009cascading}.
Cascading failures can lead to tremendous economic loss and safety concerns. 
For example, the 2003 North American blackout \cite{muir2004final} left approximately $55$ million people in black, and created about $10$ billion dollars loss.

One approach to improve the resilience of power system and mitigate cascading failures is called \emph{controlled islanding} \cite{kamali2020controlled}.
Controlled islanding deliberately trips a subset of transmission lines to partition the power system into a collection of disjoint, internally stable and connected islands.
How to partition the power system into islands has received extensive research attention. 
The islanding strategies can be computed using techniques including slow coherency-based methods \cite{yusof1993slow,you2004slow,xu2009slow}, mixed-integer linear program-based formulations \cite{kyriacou2017controlled,patsakis2019strong,teymouri2019milp,trodden2013optimization,trodden2013milp,kamali2020intentional,esmaili2020convex}, two-step spectral clustering method \cite{ding2012two}, and submodular optimization \cite{sahabandu2022submodular,liu2018controlled}.
Using the aforementioned methods, controlled islanding strategies can be synthesized to (approximately) optimize metrics such as power flow disruption, generator coherency, and load-generation imbalance.

The stability at the post-islanding operating point needs to be taken into consideration when computing the controlled islanding strategies.
Post-islanding stability-aware computation of controlled islanding strategy is non-trivial. 
For example, if a controlled islanding strategy cannot guarantee the post-islanding power flow to be within the capacity of each transmission line, controlled islanding may have to be executed again within one newly formulated island to avoid cascading failure inside the island.
In the worst-case, such bad design of controlled islanding strategies could occur recursively, leading to widely-spread blackout.
Furthermore, the controlled islanding strategy should partition the power system in a way such that the tripped connections can be re-established and thus the whole power system can be restored efficiently \cite{sarmadi2011sectionalizing,patsakis2019strong,tortos2012controlled}.
To allow efficient restoration, each island is required to have sufficient availability to black start generators. 

At present, how to compute a controlled islanding strategy that jointly (i) optimizes the widely-adopted metrics such as power flow disruption and generator coherency, and load-generation imbalance, (ii) takes post-islanding stability into consideration, and (iii) guarantees restoration after controlled islanding
has been less studied.
Such an islanding strategy cannot be readily computed by the existing approaches. 
One reason is that the computation involves both continuous variables (post-islanding power flow and load shedding at each load bus for load-generation balance) and discrete variables (choices of tripping transmission lines and allocation of blackstart generators).
Such hybrid optimization programs are generally NP-hard. 
Finding exact solutions to these programs is computationally intensive, and do not scale to large-scale power systems.
Although there exist heuristic solution algorithms to compute controlled islanding strategies \cite{zhao2003study,sun2003splitting,wang2010novel}, they omit some constraints from (i)-(iii) and cannot provide provable optimality guarantee.

In this paper, we investigate how to compute a controlled islanding strategy that jointly (i) optimizes metrics including power flow disruption, and generator coherency, (ii) considers post-islanding stability, and (iii) ensures efficient restoration of power system after islanding.
We model the post-islanding stability by ensuring that the post-islanding power flow on each transmission remain with capacity limit.
Satisfying transmission line capacity constraint ensures that the islanding strategy will not further create overflow on any transmission line and thus disrupt the formulated islands. 
In order to ensure the power system to restore efficiently after islanding, we further ensure that the islands have sufficient availability of energized black start generators and can satisfy post-islanding load-generation balance constraint.
We consider the heterogeneous load capacity and load shedding capabilities from load buses when modeling the load-generation balance constraint. 
To solve the hybrid optimization problem to compute islanding strategies, we use the concept of \emph{hybrid submodularity} in \cite{sahabandu2022hybrid} as a building block. 
We prove that the objective functions and constraints are hybrid submodular, and develop an efficient algorithm to compute the islanding strategy.
To summarize, this paper makes the following contributions.
\begin{itemize}
    \item We formulate the problem of synthesizing a controlled islanding strategy that jointly optimizes power flow disruption, dynamical stability, post-islanding stability, and blackstart generator allocation for restoration. 
    \item We translate the islanding problem to a matroid optimization problem. 
    We prove that transmission line capacity constraint for post-islanding power flow and blackstart generator allocation satisfy hybrid submodularity property.
    \item We present a local search algorithm to compute the islanding strategy.
    We develop a $\frac{1}{2}$ optimality bound for the developed algorithm based on hybrid submodularity property.
    \item We evaluate our proposed approach on \textbf{test cases. Our results show that the proposed solution approach outperforms the MILP formulate-based baseline by...}
\end{itemize}


The present paper generalizes the approach proposed in \cite{sahabandu2022hybrid} in the following aspects. 
This paper incorporates both the post-islanding stability and availability to black start generators in each island when computing controlled islanding strategies, which are not considered in \cite{sahabandu2022hybrid}.
% We consider the post-islanding operating point of the power system by ensuring that the post-islanding power flow on each transmission remain with capacity limit.
% Such guarantee ensures that the islanding strategy will not further create overflow on any transmission line and thus disrupt the formulated islands.
% In addition, we take the black start generator allocation into consideration when designing the islanding strategy. 
% The obtained islanding strategy ensures sufficient availability to black start geneartors, and hence eases the restoration process of the power system.
We prove that both constraints on transmission line capacity and black start generator allocation are hybrid supermodular in the islanding strategies, and develop and efficient solution algorithm with $\frac{1}{2}$ optimality guarantee.
We implement the proposed solution approach to large-scale power systems including \textbf{test case}.

The remainder of this paper is organized as follows.
Section \ref{sec:related} reviews related literature. 
In Section \ref{sec:background}, we present preliminary background on submodularity and matroids.
% Section \ref{sec:model} gives power system model.
Section \ref{sec:formulation} formulates the controlled islanding problem.
Section \ref{sec:sol} translates the islanding problem to a matroid optimization problem, and develops a local search algorithm based on hybrid submodularity property with $\frac{1}{2}$ optimality guarantee.
In Section \ref{sec:experiment}, we evaluate our proposed approach using \textbf{test case}.
Section \ref{sec:conclusion} concludes the paper.


==> model.tex <==
\section{System Model}\label{sec:model}

In this section, we present the system model along with notations that will be used throughout the paper.

We consider a power system and model it as a graph, denoted as $G=(\mathcal{V},\mathcal{E})$, where $\mathcal{V}$ is the set of vertices and $\mathcal{E}\subseteq\mathcal{V}\times\mathcal{V}$ is the set of edges. 
Without loss of generality, we assume that graph $G$ is connected.
Here we use the set of vertices $\mathcal{V}=\{1,\ldots,n\}$ to represent the set of buses, and use the set of edges $\mathcal{E}$ to represent the collection of transmission lines.
Among the buses, we denote the set of generator and load buses as $\mathcal{G}\subseteq \mathcal{V}$ and $\mathcal{L}\subseteq \mathcal{V}$, respectively, where $\mathcal{G}\cap\mathcal{L}=\emptyset$.
For each generator bus $j\in\mathcal{G}$, we denote its generation capacity as $\Bar{g}_j$. For each load bus $j\in\mathcal{L}$, we denote its maximum load as $\Bar{d}_j$.

For each transmission line $(j,j')\in\mathcal{E}$, we denote the power flow from bus $j$ to $j'$ through transmission line $(j,j')$ as $P_{jj'}$. 
At each bus $j\in\mathcal{V}$, the power flow satisfies the conservation law given as
\begin{equation}\label{eq:conservation}
    \sum_{j':(j,j')\in\mathcal{E}}P_{jj'}+ d_j - g_j = 0,~\forall j\in\mathcal{V}
\end{equation}
where $d_j\geq 0$ and $g_j\geq 0$ are the load and power generation at bus $j$, respectively.


To ensure reliable power system operations, we consider the following constraints in this work. 
First, the total amount of power generation should meet the total power load drawn from the grid. 
Such \emph{load-generation balance} constraint is formulated as
\begin{equation}\label{eq:balance}
    \sum_{j\in\mathcal{L}}d_j\leq \sum_{j\in\mathcal{G}}\Bar{g}_j.
\end{equation}
Second, the power generation supplied by each generator bus $j\in\mathcal{G}$ and power demand drawn from each load bus $j\in\mathcal{V}$ should satisfy
\begin{equation}
    d_j\leq \Bar{d}_j,~\forall j\in\mathcal{L}, \quad g_j\leq \Bar{g}_j,~\forall j\in\mathcal{G}.
\end{equation}
Finally, each transmission line $(j,j')$ has a capacity limit $\Bar{P}_{jj'}$. 
To avoid overflowing any transmission line in the network and creating cascading failure, we will require the following transmission line capacity constraint to hold:
\begin{equation}\label{eq:capacity}
    P_{jj'}\leq \Bar{P}_{jj'}, ~(j,j')\in\mathcal{E}.
\end{equation}
